Attributed Graph Clustering in Collaborative Settings

Graph clustering is an unsupervised machine learning method that partitions the nodes in a graph into different groups. Despite achieving significant progress in exploiting both attributed and structured data information, graph clustering methods often face practical challenges related to data isolation. Moreover, the absence of collaborative methods for graph clustering limits their effectiveness. In this paper, we propose a collaborative graph clustering framework for attributed graphs, supporting attributed graph clustering over vertically partitioned data with different participants holding distinct features of the same data. Our method leverages a novel technique that reduces the sample space, improving the efficiency of the attributed graph clustering method. Furthermore, we compare our method to its centralized counterpart under a proximity condition, demonstrating that the successful local results of each participant contribute to the overall success of the collaboration. We fully implement our approach and evaluate its utility and efficiency by conducting experiments on four public datasets. The results demonstrate that our method achieves comparable accuracy levels to centralized attributed graph clustering methods. Our collaborative graph clustering framework provides an efficient and effective solution for graph clustering challenges related to data isolation.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/attributed_graph.tex <==
\subsection{Attributed graph clustering.}
\label{sec:attributed graph clustering}

Attributed graph clustering~\cite{yang2009combining} considers the problem of combining both network structure and node content for similarity detection from networked data, such as social networks, citation networks, protein-protein interaction networks, etc. 
In particular, graph convolution~\cite{zhang2019attributed} has been demonstrated state-of-the-art performance on integrating structural and feature information. Graph convolution is defined from the perspective of graph signal processing to extract the graph topology by filtering out high-frequency noises.

% We start with introducing the Laplacian which is the classic in graph representation. 
Given an attributed non-directed graph $\mathcal{G=(V, E, X)}$, where $\mathcal{V}=\{v_1, v_2, \dots, v_n\}$ is the vertex set with $n$ nodes in total, $\mathcal{E}$ is the edge set, and $\X\in\mathbb{R}^{n\times M}$ is the feature matrix of all nodes. The symmetrically normalized graph Laplacian is defined as $L_s = I-D^{-\frac{1}{2}}AD^{-\frac{1}{2}}$, where $A$ is an adjacency matrix and $D$ is a diagonal matrix called degree matrix. $L_s$ can be eigen-decomposed as $L_s=Q\Lambda Q^{-1}$, where $\Lambda =diag(\lambda_1, \dots, \lambda_n)$ are the eigenvalues, $Q = [q_1, \dots, q_n]$ is an orthogonal matrix composed of the associated orthogonal eigenvectors. 
A linear graph filter can be represented as a matrix $G =Q p(\Lambda)Q^{-1}\in R^{n\times n}$, where $p(\Lambda) = diag(p(\lambda_1), \dots, p(\lambda_n))$
is called the frequency response function of $G$. 
% A graph signal is a real-valued vector function $f :\mathcal{V}^n  \rightarrow \mathbb{R}^n$, where $\mathcal{V}$ represent the nodes content of a graph. 
Applying this graph filter to graph signal $f :\mathcal{V}^n  \rightarrow \mathbb{R}^n$, where $\mathcal{V}$ represent the nodes content of a graph. 
Graph convolution is defined as:
$\overline{f}=Gf$, and 
$\overline{f}$ is called the filtered graph signal.

To make nearby nodes similar to each other, it has been proved~\cite{6494675} that 
% Afterwards, we introduce smoothness of a graph signal to analyze the construction of $p(\cdot)$. The smoothness of a graph signal is usually measured by Laplacian-Beltrami operator $\Omega(\cdot)$~\cite{chung1997spectral}.
% A graph signal $f$ is smooth if nearby nodes on the graph have similar features after applying the signal $f$.
% Since $Q$ is an orthogonal matrix, the eigenvectors $\{\mathbi{q}_k\}_{k=1, \dots, n}$ are a basis of the graph. A graph signal $f$ can be decomposed into a linear combination of the basis,
% \begin{equation}
% \begin{aligned}
%     f=QZ=\sum_{i=k}^{n}\mathbi{q}_kz_k,
% \end{aligned}
% \end{equation}
% where $Z=[z_1, \dots, z_n]$ are the coefficient of the basis.
% The smoothness of a basis signal $\mathbi{u}_k$ is defined as:
% \begin{equation}
% \begin{aligned}
%     \Omega(\mathbi{q}_k)=&\frac{1}{2}\sum_{(v_i, v_j)\in \mathcal{E}}a_{ij}||\frac{\mathbi{q}_{ki}}{\sqrt{d_i}}-\frac{\mathbi{q}_{kj}}{\sqrt{d_j}}||_2^2\\
%     =&\mathbi{q}_k^T L_s \mathbi{q}_k = \lambda_k,
% \end{aligned}
% \end{equation}
% where $\mathbi{u}_{ki}$ denotes the $i$-th element of $\mathbi{u}_k$, $d_i$ denotes the $i$-th element of diagonal matrix $D$. This equation shows that the smoothness of the basis signal $\mathbi{u}_k$ relies on small eigenvalue (low frequency). Since  a graph signal $f$ is a linear combination of the basis, smoother signal should contain more small eigenvalues (low frequencies) rather than large eigenvalues (high frequencies). 
% The smoothness of $\overline{f}$ is:
% \begin{equation}
%     \begin{aligned}
%     \Omega(\overline{f})&=\Omega(Gf)=\Omega(Qp(\Lambda)Q^{-1}\dot QZ)\\
%     &=\Omega(\sum_{k=1}^{n}p(\lambda_k)z_k\mathbi{q}_k)
%     =\sum_{k=1}^{n}p^2(\lambda_k)z^2_k\lambda_k
%     \end{aligned}
% \end{equation}
$p(\cdot)$ should be a nonnegative decreasing linear function.
As common practice, Laplacian smoothing filters\cite{taubin1995signal} are utilized to achieve this goal.

Generalized Laplacian smoothing filter choose $p(\lambda_i)=1-\mu\lambda_i$, where $\mu$ is a real valued constant. While $\mu=1, \frac{1}{2}, \frac{1}{\lambda_max}$ are studied in graph convolution networks(GCN) based methods, AGC~\cite{zhang2019attributed} and AGE~\cite{cui2020adaptive} respectively.

% we design an optimal filter construction.
% Setting $p(\lambda)=1-\frac{\lambda^2}{4}$, we construct a nonnegative decreasing quadratic function when $\lambda \in [0,2]$~\cite{chung1997spectral} for more efficient filter.

By performing graph convolution on the node feature matrix $\X$, we obtain the filtered feature matrix $\overline{\X} = G\X\in\mathbb{R}^{n\times M}$. 
Based on the assumption that network neighbors are more likely to be classified in the same cluster, feature matrix $\overline{\X}$ is a new data matrix that combines the graph topology and the node content.

% In the centralized setup, the participant knows the entire feature matrix $X$ and the graph $\mathcal{G=(V, E, X)}$. In this settings, many state-of-the-art works\cite{zhang2019attributed, wang2019attributed, cui2020adaptive} have been proposed.
% However, to prove the effectiveness of our solution in collaborative settings, we propose a centralized version.
% The centralized setup provide with a reasonable private base line to compare our solution which is friendly to centralized setup.

% Firstly we compute the graph filter $G$ with the graph $\mathcal{G=(V, E)}$. By applying the graph convolution on feature matrix $X\in\mathbb{R}^{n\times M}$, we obtain $\overline{X} = GX \in \in\mathbb{R}^{n\times M}$. 
% Since the filtered feature matrix $\overline{X}$ is stored by the only participant, 
% we perform the k-means on the filtered feature matrix $\overline{X}$ to partition the nodes of $\mathcal{V}$ into $K$ clusters. Protocol~\ref{alg:centralized} depicts this procedure.




==> sections/related.tex <==
\section{Related Work}

%\subsection{Horizontal federated learning}
%\label{sec:hfl}

The terminology of FL was first proposed by Google in 2017. 
It distributes the model training process of a deep neural network across multiple participants by iteratively aggregating the locally trained models into a joint global one. 
In the beginning, a parameter server initializes a model and sends it to all participants.
In each iteration, each participant trains the received model with its local data, and returns the gradients.
The parameter server aggregates the received gradients and updates the global model.
{\em Quantization}~\cite{konevcny2016federated, lin2017deep} is a way to reduce the communication overhead of Google's proposal.
The idea is to have each participant send an efficient representation of the model without affecting much of the utility.
%the client quantize the model parameter and send an efficient representation of the model.
For example, one quatization algorithm is to reduce the requirement of full (or floating point) arithmetic precision to a bit or few bits~\cite{Suresh:2017:DME:3305890.3306025}.

FL also brings new security and privacy risks.
%A backdoor can be injected to the global model to make it achieve high accuracy on both its main task and the backdoor subtask.
%A naive approach is to have the attacker train the local model with poisoned local data, which is called {\em data poisoning attacks}.
%However, the server-side aggregation can cancel out the poisoned inputs and the global model quickly forgets the backdoor.
A compromised participant can directly manipulate its gradients to 
inject a backdoor to the global model to make it achieve high accuracy on both its main task and the backdoor subtask~\cite{backdoor}.
%make the backdoor more difficult to be detected, which is called {\em model poisoning attacks}~\cite{backdoor}.
%It has been shown that such model poisoning attack is much more effective than data poisoning.
In privacy perspective, a compromised participant can infer properties of others' training data by using multi-task learning to extends her local model with an augmented property classifier connected to the last layer~\cite{Melis}.


Google's proposal {\em cannot} be directly applied to vertical FL, where participants have different feature spaces so that they cannot train models locally.
Hardy et al.~\cite{Hardy2017PrivateFL} propose a solution to run logistic regression over vertically partitioned data.
Participants compute their partial gradients locally and use homomorphic encryption to combine them.
%reword
In another work named FDML~\cite{FDML}, each participant trains a separate model using its own feature space and shares the prediction result to others (through a central server).
A central server aggregates the prediction results; all participants update their models based on the aggregated result and move to the next round.
FDML involves no cryptographic operation, but requires all participants to know the labels to train models locally, which is unrealistic in real-world.
Usually, only a single participant holds the labels and other participants only have the features.
%--------------


Existing work on FL only focuses on supervised learning and 
less attention has been paid to unsupervised learning such as $k$-means clustering.
To the best of our knowledge, all existing solutions for 
federated $k$-means clustering are fully based on cryptography~\cite{10.1145/1315245.1315306, 10.1145/1081870.1081942, DBLP:journals/popets/MohasselRT20} and they are extremely expensive.


% For example, the core idea of~\cite{10.1145/1315245.1315306} is to have two participants secret-share their data and run the $k$-means algorithm on the secret-shared data.
% However, the protocol is too slow to be used in practice:
% {\em it requires %both $O(N)$ communication complexity and 
% $O(N)$ expensive cryptographic operations} (where $N$ is the size of the sample space).
% We aim to minimize the number of cryptographic operations.






